Deep Learning Across Games

We train two neural networks adversarially to play static games. At each iteration, a row and column network observe a new random bimatrix game and output individual mixed strategies. The parameters of each network are independently updated via stochastic gradient descent on a loss defined by the individual squared regret experienced in the game. Simulations show the joint behavior of the trained networks approximates a Nash equilibrium in all games. In $2\times2$ games with multiple equilibria, the networks select the risk dominant equilibrium. These findings, which are robust and generalise out-of-distribution, illustrate how equilibrium emerges from learning across heterogeneous games.

==> tables/networks_larger.tex <==
\begin{tabular}{ccc}
\multicolumn{3}{c}{\textbf{$\mathbf{4 \times 4}$  Games [MF]}} \\[2pt]
\toprule
\textbf{Network} & \textbf{Data} & \textbf{Optimization} \\
\midrule
$L=8$ & $G^i \sim \text{Uniform}(\mathcal{G}_2)$ & $\mathcal{L}^i(G,\sigma_i,\sigma{-i}) = -R(G^i,\sigma_i,\sigma_{-i})^2/2$ \\
$D=1024$ & $K= 1\,073\,741\,824$ &  T = 8\,388\,608  \\
 $\#w = 8\,408\,066$ & B = 128 & $\eta_0=1$\\
 & &  $\alpha = 0.999999$ \\
\bottomrule
\end{tabular}

\medskip
\medskip

\begin{tabular}{ccc}
\multicolumn{3}{c}{\textbf{$\mathbf{5 \times 5}$  Games [MF]}} \\[2pt]
\toprule
\textbf{Network} & \textbf{Data} & \textbf{Optimization} \\
\midrule
$L=8$ & $G^i \sim \text{Uniform}(\mathcal{G}_3)$ & $\mathcal{L}^i(G,\sigma_i,\sigma{-i}) = -R(G^i,\sigma_i,\sigma_{-i})^2/2$ \\
$D=2048$ & $K= 2\,147\,483\,648$ & T = 8\,388\,608 \\
$\#w = 33\,615\,875$ & B = 256 & $\eta_0=1$\\
 & &  $\alpha = 0.9999995$ \\
\bottomrule
\end{tabular}

